Neural Approximation of an Auto-Regressive Process through Confidence Guided Sampling

We propose a generic confidence-based approximation that can be plugged in and simplify the auto-regressive generation process with a proved convergence. We first assume that the priors of future samples can be generated in an independently and identically distributed (i.i.d.) manner using an efficient predictor. Given the past samples and future priors, the mother AR model can post-process the priors while the accompanied confidence predictor decides whether the current sample needs a resampling or not. Thanks to the i.i.d. assumption, the post-processing can update each sample in a parallel way, which remarkably accelerates the mother model. Our experiments on different data domains including sequences and images show that the proposed method can successfully capture the complex structures of the data and generate the meaningful future samples with lower computational cost while preserving the sequential relationship of the data.

==> 8_Algorithm.tex <==
%----------------------------------------------------------------------------------
\begin{algorithm} [h]
\caption{Training procedure of the Skim-PixelCNN.}
\begin{algorithmic}[1]
\Require 
%Pre-trained encoder CNN (\(W_{C}\)), 
Training image $(\textbf{x}^{(i)}), i= 1...N$
%ground truths \(\{l_{i}\}\) and 
\State Initialize network parameters $\theta_0$, $W_0$, and $V_0$. 
\Repeat 
	\State $v^{(i)}\sim Uniform([1, n^2])$.
    \State $k^{(i)} = v^{(i)} + l^{(i)}$, ~$l^{(i)} = \min{(K, n^2-v^{(i)})}$.    
    \State $\mathbf{\tilde{x}}^{(i)}_{k^{(i)}:v^{(i)}} \sim p_\theta({\mathbf{x}^{(i)}_{k^{(i)}:v^{(i)}}}| \mathbf{x}^{(i)}_{\leq k^{(i)}})$.
    \State $\mathbf{z}^{(i)}_{k^{(i)}:v^{(i)}} \sim f_W(\mathbf{x}^{(i)}_{\leq k^{(i)}})$.
    \State $\mathbf{f}^{(i)}_{k^{(i)}:v^{(i)}} = q_{\theta,W}(\cdot|\mathbf{x}^{(i)}_{\leq k^{(i)}})$.
    \State $\mathbf{f}^{(i)(d)}_{k^{(i)}:v^{(i)}} \leftarrow \mathbf{f}^{(i)}_{k^{(i)}:v^{(i)}}$ by equation (8).
    
	\State Update $\theta, W$ by equation (10) using $\mathbf{\tilde{x}}^{(i)}_{k^{(i)}:v^{(i)}}, \mathbf{z}^{(i)}_{k^{(i)}:v^{(i)}}$.
    \State Update $V$ by equation (9) using $\mathbf{f}^{(i)(d)}_{k^{(i)}:v^{(i)}}$.
    
    
%     \State \(\Delta W_{RL} \propto \sum_{l=1}^\mathcal{L} \sum_{t=1}^{T_l}  \frac{\partial \log p(a_{t,l}|s_{t,l};W_{RL})}{\partial W_{RL}} z_{t,l}\)~\cite{williams1992simple_REINFORCE}
\Until{ converge}
% \algrule
\end{algorithmic}
\label{algo:training}
\end{algorithm}

%----------------------------------------------------------------------------------
\begin{algorithm} [h]
\caption{Inference procedure of the Skim-PixelCNN.}
\begin{algorithmic}[1]
\Require Trained network parameters $\theta, W, V$.
%Pre-trained encoder CNN (\(W_{C}\)), 
%ground truths \(\{l_{i}\}\) and 
\State Initialize empty image $d(i) = 0, i\in[1,R*C]$.
\State $i=1.$
\State
\State $\#$ Generate Anchor images
\State Set $d[1]$ randomly.
\Repeat 	
	\State $d[i+1] \sim p_\theta(x|d[\leq i])$.
    \State $i \leftarrow i + 1$.   
%     \State \(\Delta W_{RL} \propto \sum_{l=1}^\mathcal{L} \sum_{t=1}^{T_l}  \frac{\partial \log p(a_{t,l}|s_{t,l};W_{RL})}{\partial W_{RL}} z_{t,l}\)~\cite{williams1992simple_REINFORCE}
\Until{$i \leq A$} ($4*C$ in the paper), 
\State
\State $\#$ Skim-PixelCNN inference
\Repeat 
\If{$\mod(i,C) == 0$}
\State Set $l = min(K, n^2-i)$.
\State $p[i+l:i] = f_W(d[\leq i])$.
\State $c[i+l:i] = g_V(p[i+l:i])$.
\EndIf
\State $k \leftarrow 1$
\Repeat 
\If{$c[i+k] < \eps$}
\State $d[i+k] \sim p_\theta(x|d[\leq i+k])$.
\Else
\State $d[i+k] = p[i+k]$.
\EndIf
\State $k\leftarrow k + 1$.
\Until{$k \leq l$}
\State $i \leftarrow k + k$
\Until{$i \leq R*C$}
% \algrule
\end{algorithmic}
\label{algo:Inference}
\end{algorithm}


\section{Implementation Details}
To supplement the explanation for the training and inference of the proposed Skim-PixelCNN, this section presents the pseudo-codes of the processes in Algorithm~(\ref{algo:training}) and ~(\ref{algo:Inference}).
In Algorithm~(\ref{algo:training}), the term $\mathbf{f}^{(i)(d)}_{k^{(i)}:v^{(i)}}$ denotes the binary decision vector for the image region $\mathbf{x}^{(i)}_{k^{(i)}:v^{(i)}}$. See Section 3 for other notations and equations. 
The operations in line $14$ to $18$ describe the prediction procedure for skimming. 
We confirmed from the experiments that it is enough to update the prediction results for each row.
We note that the index $i$ searches every $RC$ number of pixels, and conduct PixelCNN inference for every pixel if no skimming occurred.

\section{Supplementary Explanation on the Proposed Approximation}
In this section, we show that the cost function of the Skim-PixelCNN is a regularized version of the original PixelCNN. At the extremum, the approximated pixel distribution Skim-PixelCNN is equivalent to that of the original PixelCNN. In Skim-PixelCNN, our approximate distribution $q(\mathbf{x}_{j+1:i}|\mathbf{x}_{\leq i}, \mathbf{z}_{j:i})$ can be reformulated as follows:
\begin{align} 
\label{eq:pixCNN_app}
&q_{\phi,\theta}(\mathbf{x}_{j+1:i}|\mathbf{x}_{\leq i}, \mathbf{z}_{j:i}) \equiv p_\theta(x_{i+1}|\mathbf{x}_{\leq i})\prod^{j+1}_{l=i+2}{q_\phi(x_l|\mathbf{x}_{\leq i}, z_{i+1},...,z_{l-1})}\\
&= \frac{p_\theta(\mathbf{x}_{\leq i+1})}{p_\theta(\mathbf{x}_{\leq i})}\cdot
\frac{q_\phi(\mathbf{x}_{\leq i},z_{i+1},x_{i+2})}{q_\phi(\mathbf{x}_{\leq i}, z_{i+1})}\cdot
,\cdots,\cdot 
\frac{q_\phi(\mathbf{x}_{\leq i},\mathbf{z}_{j-1:i},x_{j})}{q_\phi(\mathbf{x}_{\leq i}, \mathbf{z}_{j-1:i})} \cdot
\frac{q_\phi(\mathbf{x}_{\leq i},\mathbf{z}_{j:i},x_{j+1})}{q_\phi(\mathbf{x}_{\leq i}, \mathbf{z}_{j:i})}\\
&= \underbrace{\frac{p_\theta(\mathbf{x}_{\leq i+1})}{p_\theta(\mathbf{x}_{\leq i})}\cdot 
\frac{p_\theta(\mathbf{x}_{\leq i+2})}{p_\theta(\mathbf{x}_{\leq i+1})}\cdot, \cdots, \cdot
\frac{p_\theta(\mathbf{x}_{\leq j+1})}{p_\theta(\mathbf{x}_{\leq j})}}_{p_{\theta}(\mathbf{x}_{j+1:i}|\mathbf{x}_{\leq i})} \cdot 
\underbrace{\left[\frac{p_\theta(\mathbf{x}_{\leq i+1})}{q_\phi(\mathbf{x}_{\leq i},z_{i+1})}\cdot, \cdots, \cdot \frac{q_\phi(\mathbf{x}_{\leq i},\mathbf{z}_{j:i},x_{j+1})}{p_\theta(\mathbf{x}_{\leq j+1})}
\right]}_{\mathcal{R}(p_\theta, q_\phi, \mathbf{z}_{j:i})}
\end{align}
Therefore, our proposed cost function can be represented as the negative log-likelihood of the PixelCNN with a regularizer $-\log\mathcal{R}(p_\theta, q_\phi, z_{j:i})$:
\begin{equation} 
\label{eq:regmin}
\min_{\phi,\theta}-\mathbb{E}_{p_\theta(\mathbf{x}_{j+1:i}|\mathbf{x}_{\leq i})}[\log p_{\theta}(\mathbf{x}_{j+1:i}|\mathbf{x}_{\leq i}))+\log\mathcal{R}(p_\theta, q_\phi, \mathbf{z}_{j:i})]
\end{equation}
Note that the proposed cost function is equivalent to that of the original PixelCNN when $\log\mathcal{R}(p_\theta, q_\phi, \mathbf{z}_{j:i})=0$, which is true under the condition of $\mathbf{z}_{j:i} = \mathbf{x}_{j:i}$ and $q_\phi(\cdot | \cdot)=p_\theta(\cdot | \cdot)$. Here, $\mathbf{z}_{j:i}=f_W(\mathbf{x}_{\leq i})$.
% Since $\mathcal{R}(p_\theta, q_\phi, \mathbf{z}_{j:i})=\left[\frac{p_\theta(\mathbf{x}_{\leq i+1})}{q_\phi(\mathbf{x}_{\leq i},z_{i+1})}\cdot, \cdots, \cdot \frac{q_\phi(\mathbf{x}_{\leq i},\mathbf{z}_{j:i},x_{j+1})}{p_\theta(\mathbf{x}_{\leq j+1})}
% \right]$
By minimizing the equation \eqref{eq:regmin}, $\mathcal{R}(p_\theta, q_\phi, \mathbf{z}_{j:i})$ enforces the direction of the optimization to estimate the probability ratio of $q_\phi$ and $p_\theta$ while it minimize the gap between $\frac{q_\phi(\mathbf{x}_{\leq i},\mathbf{z}_{j:i},x_{j+1})}{q_\phi(\mathbf{x}_{\leq i}, \mathbf{z}_{j:i})}$ so that $\mathbf{z}_{j:i} = f_W(\mathbf{x}_{\leq i})$ approaches to $\mathbf{x}_{j:i}$.
 

